Discrete Infomax Codes for Supervised Representation Learning

Learning compact discrete representations of data is a key task on its own or for facilitating subsequent processing of data. In this paper we present a model that produces Discrete InfoMax Codes (DIMCO); we learn a probabilistic encoder that yields k-way d-dimensional codes associated with input data. Our model's learning objective is to maximize the mutual information between codes and labels with a regularization, which enforces entries of a codeword to be as independent as possible. We show that the infomax principle also justifies previous loss functions (e.g., cross-entropy) as its special cases. Our analysis also shows that using shorter codes, as DIMCO does, reduces overfitting in the context of few-shot classification. Through experiments in various domains, we observe this implicit meta-regularization effect of DIMCO. Furthermore, we show that the codes learned by DIMCO are efficient in terms of both memory and retrieval time compared to previous methods.

==> __latexindent_temp.tex <==

@InProceedings{Lee2018,
  author        = {Yoonho Lee and Seungjin Choi},
  title         = {Gradient-Based Meta-Learning with Learned Layerwise Metric and Subspace},
  booktitle = {Proceedings of the International Conference on Machine Learning},
  year          = 2018
}

@Article{grover2017flow,
  author  = {Grover, Aditya and Dhar, Manik and Ermon, Stefano},
  title   = {Flow-GAN: Combining maximum likelihood and adversarial learning in generative models},
  journal = {arXiv preprint arXiv:1705.08868},
  year    = {2017},
}

@Article{finn2017model,
  author  = {Finn, Chelsea and Abbeel, Pieter and Levine, Sergey},
  title   = {Model-agnostic meta-learning for fast adaptation of deep networks},
  journal = {arXiv preprint arXiv:1703.03400},
  year    = {2017},
}

@Article{finn2017meta,
  author  = {Finn, Chelsea and Levine, Sergey},
  title   = {Meta-learning and universality: Deep representations and gradient descent can approximate any learning algorithm},
  journal = {arXiv preprint arXiv:1710.11622},
  year    = {2017},
}

@Article{nichol2018reptile,
  author  = {Nichol, Alex and Schulman, John},
  title   = {Reptile: a Scalable Metalearning Algorithm},
  journal = {arXiv preprint arXiv:1803.02999},
  year    = {2018},
}

@InProceedings{snell2017prototypical,
  author    = {Snell, Jake and Swersky, Kevin and Zemel, Richard},
  title     = {Prototypical networks for few-shot learning},
  booktitle = {Advances in Neural Information Processing Systems},
  year      = {2017},
  pages     = {4077--4087},
}

@InProceedings{hoffer2015deep,
  author       = {Hoffer, Elad and Ailon, Nir},
  title        = {Deep metric learning using triplet network},
  booktitle    = {International Workshop on Similarity-Based Pattern Recognition},
  year         = {2015},
  pages        = {84--92},
  organization = {Springer},
}

@InProceedings{wu2017sampling,
  author    = {Wu, Chao-Yuan and Manmatha, R and Smola, Alexander J and Krahenbuhl, Philipp},
  title     = {Sampling matters in deep embedding learning},
  booktitle = {Proceedings of the IEEE International Conference on Computer Vision},
  year      = {2017},
  pages     = {2840--2848},
}

@InProceedings{duan2018deep,
  author    = {Duan, Yueqi and Zheng, Wenzhao and Lin, Xudong and Lu, Jiwen and Zhou, Jie},
  title     = {Deep Adversarial Metric Learning},
  booktitle = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  year      = {2018},
  pages     = {2780--2789},
}

@InProceedings{oh2016deep,
  author    = {Oh Song, Hyun and Xiang, Yu and Jegelka, Stefanie and Savarese, Silvio},
  title     = {Deep metric learning via lifted structured feature embedding},
  booktitle = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  year      = {2016},
  pages     = {4004--4012},
}

@InProceedings{sohn2016improved,
  author    = {Sohn, Kihyuk},
  title     = {Improved deep metric learning with multi-class n-pair loss objective},
  booktitle = {Advances in Neural Information Processing Systems},
  year      = {2016},
  pages     = {1857--1865},
}

@inproceedings{movshovitz2017no,
  title={No fuss distance metric learning using proxies},
  author={Movshovitz-Attias, Yair and Toshev, Alexander and Leung, Thomas K and Ioffe, Sergey and Singh, Saurabh},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={360--368},
  year={2017}
}

@Article{belghazi2018mine,
  author  = {Belghazi, Mohamed Ishmael and Baratin, Aristide and Rajeswar, Sai and Ozair, Sherjil and Bengio, Yoshua and Courville, Aaron and Hjelm, R Devon},
  title   = {MINE: mutual information neural estimation},
  journal = {arXiv preprint arXiv:1801.04062},
  year    = {2018},
}

@Article{hjelm2018learning,
  author  = {Hjelm, R Devon and Fedorov, Alex and Lavoie-Marchildon, Samuel and Grewal, Karan and Trischler, Adam and Bengio, Yoshua},
  title   = {Learning deep representations by mutual information estimation and maximization},
  journal = {arXiv preprint arXiv:1808.06670},
  year    = {2018},
}

@Article{bell1995information,
  author    = {Bell, Anthony J and Sejnowski, Terrence J},
  title     = {An information-maximization approach to blind separation and blind deconvolution},
  journal   = {Neural computation},
  year      = {1995},
  volume    = {7},
  number    = {6},
  pages     = {1129--1159},
  publisher = {MIT Press},
}

@Article{linsker1988self,
  author    = {Linsker, Ralph},
  title     = {Self-organization in a perceptual network},
  journal   = {Computer},
  year      = {1988},
  volume    = {21},
  number    = {3},
  pages     = {105--117},
  publisher = {IEEE},
}

@InProceedings{vinyals2016matching,
  author    = {Vinyals, Oriol and Blundell, Charles and Lillicrap, Timothy and Wierstra, Daan and others},
  title     = {Matching networks for one shot learning},
  booktitle = {Advances in neural information processing systems},
  year      = {2016},
  pages     = {3630--3638},
}

@Article{donsker1983asymptotic,
  author    = {Donsker, Monroe D and Varadhan, SR Srinivasa},
  title     = {Asymptotic evaluation of certain Markov process expectations for large time. IV},
  journal   = {Communications on Pure and Applied Mathematics},
  year      = {1983},
  volume    = {36},
  number    = {2},
  pages     = {183--212},
  publisher = {Wiley Online Library},
}

@Article{tishby2000information,
  author  = {Tishby, Naftali and Pereira, Fernando C and Bialek, William},
  title   = {The information bottleneck method},
  journal = {arXiv preprint physics/0004057},
  year    = {2000},
}

@Article{shwartz2017opening,
  author  = {Shwartz-Ziv, Ravid and Tishby, Naftali},
  title   = {Opening the black box of deep neural networks via information},
  journal = {arXiv preprint arXiv:1703.00810},
  year    = {2017},
}

@Book{cover2012elements,
  title     = {Elements of information theory},
  publisher = {John Wiley \& Sons},
  year      = {2012},
  author    = {Cover, Thomas M and Thomas, Joy A},
}

@Article{jang2016categorical,
  author  = {Jang, Eric and Gu, Shixiang and Poole, Ben},
  title   = {Categorical reparameterization with gumbel-softmax},
  journal = {arXiv preprint arXiv:1611.01144},
  year    = {2016},
}

@Article{maddison2016concrete,
  author  = {Maddison, Chris J and Mnih, Andriy and Teh, Yee Whye},
  title   = {The concrete distribution: A continuous relaxation of discrete random variables},
  journal = {arXiv preprint arXiv:1611.00712},
  year    = {2016},
}

@InProceedings{mcallester1999pac,
  author       = {McAllester, David A},
  title        = {PAC-Bayesian model averaging},
  booktitle    = {COLT},
  year         = {1999},
  volume       = {99},
  pages        = {164--170},
  organization = {Citeseer},
}

@Book{shalev2014understanding,
  title     = {Understanding machine learning: From theory to algorithms},
  publisher = {Cambridge university press},
  year      = {2014},
  author    = {Shalev-Shwartz, Shai and Ben-David, Shai},
}

@Article{shamir2010learning,
  author    = {Shamir, Ohad and Sabato, Sivan and Tishby, Naftali},
  title     = {Learning and generalization with the information bottleneck},
  journal   = {Theoretical Computer Science},
  year      = {2010},
  volume    = {411},
  number    = {29-30},
  pages     = {2696--2711},
  publisher = {Elsevier},
}

@InProceedings{tishby2015deep,
  author       = {Tishby, Naftali and Zaslavsky, Noga},
  title        = {Deep learning and the information bottleneck principle},
  booktitle    = {2015 IEEE Information Theory Workshop (ITW)},
  year         = {2015},
  pages        = {1--5},
  organization = {IEEE},
}

@Article{goyal2019infobot,
  author  = {Goyal, Anirudh and Islam, Riashat and Strouse, Daniel and Ahmed, Zafarali and Botvinick, Matthew and Larochelle, Hugo and Levine, Sergey and Bengio, Yoshua},
  title   = {InfoBot: Transfer and Exploration via the Information Bottleneck},
  journal = {arXiv preprint arXiv:1901.10902},
  year    = {2019},
}

@Article{amit2017meta,
  author  = {Amit, Ron and Meir, Ron},
  title   = {Meta-learning by Adjusting Priors Based on Extended PAC-Bayes Theory},
  journal = {arXiv preprint arXiv:1711.01244},
  year    = {2017},
}

@InProceedings{ravi2018amortized,
  author    = {Sachin Ravi and Alex Beatson},
  title     = {Amortized Bayesian Meta-Learning},
  booktitle = {International Conference on Learning Representations},
  year      = {2019},
  url       = {https://openreview.net/forum?id=rkgpy3C5tX},
}

@Article{alemi2016deep,
  author  = {Alemi, Alexander A and Fischer, Ian and Dillon, Joshua V and Murphy, Kevin},
  title   = {Deep Variational Information Bottleneck},
  journal = {arXiv preprint arXiv:1612.00410},
  year    = {2016},
}

@Article{alemi2017fixing,
  author  = {Alemi, Alexander A and Poole, Ben and Fischer, Ian and Dillon, Joshua V and Saurous, Rif A and Murphy, Kevin},
  title   = {Fixing a Broken ELBO},
  journal = {arXiv preprint arXiv:1711.00464},
  year    = {2017},
}

@InProceedings{hu2017learning,
  author       = {Hu, Weihua and Miyato, Takeru and Tokui, Seiya and Matsumoto, Eiichi and Sugiyama, Masashi},
  title        = {Learning discrete representations via information maximizing self-augmented training},
  booktitle    = {Proceedings of the 34th International Conference on Machine Learning-Volume 70},
  year         = {2017},
  pages        = {1558--1567},
  organization = {JMLR. org},
}

@Article{slonim2005information,
  author    = {Slonim, Noam and Atwal, Gurinder Singh and Tka{\v{c}}ik, Ga{\v{s}}per and Bialek, William},
  title     = {Information-based clustering},
  journal   = {Proceedings of the National Academy of Sciences},
  year      = {2005},
  volume    = {102},
  number    = {51},
  pages     = {18297--18302},
  publisher = {National Acad Sciences},
}

@Article{jegou2011product,
  author    = {Jegou, Herve and Douze, Matthijs and Schmid, Cordelia},
  title     = {Product quantization for nearest neighbor search},
  journal   = {IEEE transactions on pattern analysis and machine intelligence},
  year      = {2011},
  volume    = {33},
  number    = {1},
  pages     = {117--128},
  publisher = {IEEE},
}

@InProceedings{vaswani2017attention,
  author    = {Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia},
  title     = {Attention is all you need},
  booktitle = {Advances in neural information processing systems},
  year      = {2017},
  pages     = {5998--6008},
}

@InProceedings{norouzi2013cartesian,
  author    = {Norouzi, Mohammad and Fleet, David J},
  title     = {Cartesian k-means},
  booktitle = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  year      = {2013},
  pages     = {3017--3024},
}

@Article{rusu2018meta,
  author  = {Rusu, Andrei A and Rao, Dushyant and Sygnowski, Jakub and Vinyals, Oriol and Pascanu, Razvan and Osindero, Simon and Hadsell, Raia},
  title   = {Meta-learning with latent embedding optimization},
  journal = {arXiv preprint arXiv:1807.05960},
  year    = {2018},
}

@InProceedings{oreshkin2018tadam,
  author    = {Oreshkin, Boris and L{\'o}pez, Pau Rodr{\'\i}guez and Lacoste, Alexandre},
  title     = {Tadam: Task dependent adaptive metric for improved few-shot learning},
  booktitle = {Advances in Neural Information Processing Systems},
  year      = {2018},
  pages     = {721--731},
}

@Article{zintgraf2018caml,
  author  = {Zintgraf, Luisa M and Shiarlis, Kyriacos and Kurin, Vitaly and Hofmann, Katja and Whiteson, Shimon},
  title   = {CAML: Fast Context Adaptation via Meta-Learning},
  journal = {arXiv preprint arXiv:1810.03642},
  year    = {2018},
}

@Article{kingma2014adam,
  author  = {Kingma, Diederik P and Ba, Jimmy},
  title   = {Adam: A method for stochastic optimization},
  journal = {arXiv preprint arXiv:1412.6980},
  year    = {2014},
}

@InProceedings{krizhevsky2012imagenet,
  author    = {Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
  title     = {Imagenet classification with deep convolutional neural networks},
  booktitle = {Advances in neural information processing systems},
  year      = {2012},
  pages     = {1097--1105},
}

@InProceedings{sung2018learning,
  author    = {Sung, Flood and Yang, Yongxin and Zhang, Li and Xiang, Tao and Torr, Philip HS and Hospedales, Timothy M},
  title     = {Learning to compare: Relation network for few-shot learning},
  booktitle = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  year      = {2018},
  pages     = {1199--1208},
}

@InProceedings{koch2015siamese,
  author    = {Koch, Gregory and Zemel, Richard and Salakhutdinov, Ruslan},
  title     = {Siamese neural networks for one-shot image recognition},
  booktitle = {ICML deep learning workshop},
  year      = {2015},
  volume    = {2},
}

@Article{strouse2017deterministic,
  author    = {Strouse, DJ and Schwab, David J},
  title     = {The deterministic information bottleneck},
  journal   = {Neural computation},
  year      = {2017},
  volume    = {29},
  number    = {6},
  pages     = {1611--1630},
  publisher = {MIT Press},
}

@InProceedings{chen2016infogan,
  author    = {Chen, Xi and Duan, Yan and Houthooft, Rein and Schulman, John and Sutskever, Ilya and Abbeel, Pieter},
  title     = {Infogan: Interpretable representation learning by information maximizing generative adversarial nets},
  booktitle = {Advances in neural information processing systems},
  year      = {2016},
  pages     = {2172--2180},
}

@InProceedings{van2017neural,
  author    = {van den Oord, Aaron and Vinyals, Oriol and others},
  title     = {Neural discrete representation learning},
  booktitle = {Advances in Neural Information Processing Systems},
  year      = {2017},
  pages     = {6306--6315},
}

@Article{shannon1948mathematical,
  author    = {Shannon, Claude Elwood},
  title     = {A mathematical theory of communication},
  journal   = {Bell system technical journal},
  year      = {1948},
  volume    = {27},
  number    = {3},
  pages     = {379--423},
  publisher = {Wiley Online Library},
}

@Article{jeong2018efficient,
  author  = {Jeong, Yeonwoo and Song, Hyun Oh},
  title   = {Efficient end-to-end learning for quantizable representations},
  journal = {arXiv preprint arXiv:1805.05809},
  year    = {2018},
}

@Article{rolfe2016discrete,
  author  = {Rolfe, Jason Tyler},
  title   = {Discrete variational autoencoders},
  journal = {arXiv preprint arXiv:1609.02200},
  year    = {2016},
}

@Article{ravi2016optimization,
  author = {Ravi, Sachin and Larochelle, Hugo},
  title  = {Optimization as a model for few-shot learning},
  year   = {2016},
}

@Article{wah2011caltech,
  author    = {Wah, Catherine and Branson, Steve and Welinder, Peter and Perona, Pietro and Belongie, Serge},
  title     = {The caltech-ucsd birds-200-2011 dataset},
  year      = {2011},
  publisher = {California Institute of Technology},
}

@Article{liu2018transductive,
  author  = {Liu, Yanbin and Lee, Juho and Park, Minseop and Kim, Saehoon and Yang, Yi},
  title   = {Transductive propagation network for few-shot learning},
  journal = {arXiv preprint arXiv:1805.10002},
  year    = {2018},
}

@Article{mishra2017simple,
  author  = {Mishra, Nikhil and Rohaninejad, Mostafa and Chen, Xi and Abbeel, Pieter},
  title   = {A simple neural attentive meta-learner},
  journal = {arXiv preprint arXiv:1707.03141},
  year    = {2017},
}

@InProceedings{szegedy2015going,
  author    = {Szegedy, Christian and Liu, Wei and Jia, Yangqing and Sermanet, Pierre and Reed, Scott and Anguelov, Dragomir and Erhan, Dumitru and Vanhoucke, Vincent and Rabinovich, Andrew},
  title     = {Going deeper with convolutions},
  booktitle = {Proceedings of the IEEE conference on computer vision and pattern recognition},
  year      = {2015},
  pages     = {1--9},
}

@Article{ioffe2015batch,
  author  = {Ioffe, Sergey and Szegedy, Christian},
  title   = {Batch normalization: Accelerating deep network training by reducing internal covariate shift},
  journal = {arXiv preprint arXiv:1502.03167},
  year    = {2015},
}

@InProceedings{chen2018isolating,
  author    = {Chen, Tian Qi and Li, Xuechen and Grosse, Roger B and Duvenaud, David K},
  title     = {Isolating sources of disentanglement in variational autoencoders},
  booktitle = {Advances in Neural Information Processing Systems},
  year      = {2018},
  pages     = {2610--2620},
}

@Article{oord2018representation,
  author  = {Oord, Aaron van den and Li, Yazhe and Vinyals, Oriol},
  title   = {Representation learning with contrastive predictive coding},
  journal = {arXiv preprint arXiv:1807.03748},
  year    = {2018},
}

@Article{flennerhag2018transferring,
  author  = {Flennerhag, Sebastian and Moreno, Pablo G and Lawrence, Neil D and Damianou, Andreas},
  title   = {Transferring knowledge across learning processes},
  journal = {arXiv preprint arXiv:1812.01054},
  year    = {2018},
}

@Article{metz2018meta,
  author  = {Metz, Luke and Maheswaranathan, Niru and Cheung, Brian and Sohl-Dickstein, Jascha},
  title   = {Meta-Learning Update Rules for Unsupervised Representation Learning},
  journal = {arXiv preprint arXiv:1804.00222},
  year    = {2018},
}

@Article{triantafillou2019meta,
  author  = {Triantafillou, Eleni and Zhu, Tyler and Dumoulin, Vincent and Lamblin, Pascal and Xu, Kelvin and Goroshin, Ross and Gelada, Carles and Swersky, Kevin and Manzagol, Pierre-Antoine and Larochelle, Hugo},
  title   = {Meta-dataset: A dataset of datasets for learning to learn from few examples},
  journal = {arXiv preprint arXiv:1903.03096},
  year    = {2019},
}

@Article{razavi2019generating,
  author  = {Razavi, Ali and Oord, Aaron van den and Vinyals, Oriol},
  title   = {Generating Diverse High-Fidelity Images with VQ-VAE-2},
  journal = {arXiv preprint arXiv:1906.00446},
  year    = {2019},
}

@Article{grover2018uncertainty,
  author  = {Grover, Aditya and Ermon, Stefano},
  title   = {Uncertainty autoencoders: Learning compressed representations via variational information maximization},
  journal = {arXiv preprint arXiv:1812.10539},
  year    = {2018},
}

@InProceedings{choi2019neural,
  author    = {Choi, Kristy and Tatwawadi, Kedar and Grover, Aditya and Weissman, Tsachy and Ermon, Stefano},
  title     = {Neural Joint Source-Channel Coding},
  booktitle = {International Conference on Machine Learning},
  year      = {2019},
  pages     = {1182--1192},
}

@Article{kim2018bayesian,
  author  = {Kim, Taesup and Yoon, Jaesik and Dia, Ousmane and Kim, Sungwoong and Bengio, Yoshua and Ahn, Sungjin},
  title   = {Bayesian model-agnostic meta-learning},
  journal = {arXiv preprint arXiv:1806.03836},
  year    = {2018},
}

@Article{hamming1950error,
  author    = {Hamming, Richard W},
  title     = {Error detecting and error correcting codes},
  journal   = {The Bell system technical journal},
  year      = {1950},
  volume    = {29},
  number    = {2},
  pages     = {147--160},
  publisher = {Nokia Bell Labs},
}

@Article{yin2019meta,
  author  = {Yin, Mingzhang and Tucker, George and Zhou, Mingyuan and Levine, Sergey and Finn, Chelsea},
  title   = {Meta-Learning without Memorization},
  journal = {arXiv preprint arXiv:1912.03820},
  year    = {2019},
}

@Article{gray1998quantization,
  author    = {Gray, Robert M. and Neuhoff, David L.},
  title     = {Quantization},
  journal   = {IEEE transactions on information theory},
  year      = {1998},
  volume    = {44},
  number    = {6},
  pages     = {2325--2383},
  publisher = {IEEE},
}

@Article{gong2012iterative,
  author    = {Gong, Yunchao and Lazebnik, Svetlana and Gordo, Albert and Perronnin, Florent},
  title     = {Iterative quantization: A procrustean approach to learning binary codes for large-scale image retrieval},
  journal   = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
  year      = {2012},
  volume    = {35},
  number    = {12},
  pages     = {2916--2929},
  publisher = {IEEE},
}

@Article{kuncheva2003measures,
  author    = {Kuncheva, Ludmila I and Whitaker, Christopher J},
  title     = {Measures of diversity in classifier ensembles and their relationship with the ensemble accuracy},
  journal   = {Machine learning},
  year      = {2003},
  volume    = {51},
  number    = {2},
  pages     = {181--207},
  publisher = {Springer},
}

@InProceedings{lee2019meta,
  author    = {Lee, Kwonjoon and Maji, Subhransu and Ravichandran, Avinash and Soatto, Stefano},
  title     = {Meta-learning with differentiable convex optimization},
  booktitle = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  year      = {2019},
  pages     = {10657--10665},
}

@Article{munkhdalai2017rapid,
  author  = {Munkhdalai, Tsendsuren and Yuan, Xingdi and Mehri, Soroush and Trischler, Adam},
  title   = {Rapid adaptation with conditionally shifted neurons},
  journal = {arXiv preprint arXiv:1712.09926},
  year    = {2017},
}

@InProceedings{imagenet_cvpr09,
  author    = {Deng, J. and Dong, W. and Socher, R. and Li, L.-J. and Li, K. and Fei-Fei, L.},
  title     = {{ImageNet: A Large-Scale Hierarchical Image Database}},
  booktitle = {CVPR09},
  year      = {2009},
  bibsource = {http://www.image-net.org/papers/imagenet_cvpr09.bib},
}

@TechReport{Krizhevsky09learningmultiple,
  author = {Alex Krizhevsky},
  title  = {Learning multiple layers of features from tiny images},
  year   = {2009},
}

@InProceedings{he2016deep,
  author    = {He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  title     = {Deep residual learning for image recognition},
  booktitle = {Proceedings of the IEEE conference on computer vision and pattern recognition},
  year      = {2016},
  pages     = {770--778},
}

@InProceedings{jacob2018quantization,
  author    = {Jacob, Benoit and Kligys, Skirmantas and Chen, Bo and Zhu, Menglong and Tang, Matthew and Howard, Andrew and Adam, Hartwig and Kalenichenko, Dmitry},
  title     = {Quantization and training of neural networks for efficient integer-arithmetic-only inference},
  booktitle = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  year      = {2018},
  pages     = {2704--2713},
}

@InProceedings{KrauseStarkDengFei-Fei_3DRR2013,
  author    = {Jonathan Krause and Michael Stark and Jia Deng and Li Fei-Fei},
  title     = {3D Object Representations for Fine-Grained Categorization},
  booktitle = {4th International IEEE Workshop on 3D Representation and Recognition (3dRR-13)},
  year      = {2013},
  address   = {Sydney, Australia},
}

@Article{ye2018learning,
  author  = {Ye, Han-Jia and Hu, Hexiang and Zhan, De-Chuan and Sha, Fei},
  title   = {Learning embedding adaptation for few-shot learning},
  journal = {arXiv preprint arXiv:1812.03664},
  year    = {2018},
}

@Article{opitz2018deep,
  author    = {Opitz, Michael and Waltner, Georg and Possegger, Horst and Bischof, Horst},
  title     = {Deep metric learning with bier: Boosting independent embeddings robustly},
  journal   = {IEEE transactions on pattern analysis and machine intelligence},
  year      = {2018},
  publisher = {IEEE},
}

@Comment{jabref-meta: databaseType:bibtex;}

@article{yideep2014,
  title={Deep metric learning for practical person re-identification},
  author={Yi, D and Lei, Z and Li, SZ},
  journal={ArXiv e-prints},
  year={2014}
}

@article{ILSVRC15,
Author = {Olga Russakovsky and Jia Deng and Hao Su and Jonathan Krause and Sanjeev Satheesh and Sean Ma and Zhiheng Huang and Andrej Karpathy and Aditya Khosla and Michael Bernstein and Alexander C. Berg and Li Fei-Fei},
Title = {ImageNet Large Scale Visual Recognition Challenge},
Year = {2015},
journal   = {International Journal of Computer Vision (IJCV)},
doi = {10.1007/s11263-015-0816-y},
volume={115},
number={3},
pages={211-252}
}
